PASS: An ImageNet replacement for self-supervised pretraining without humans

Computer vision has long relied on ImageNet and other large datasets of images sampled from the Internet for pretraining models. However, these datasets have ethical and technical shortcomings, such as containing personal information taken without consent, unclear license usage, biases, and, in some cases, even problematic image content. On the other hand, state-of-the-art pretraining is nowadays obtained with unsupervised methods, meaning that labelled datasets such as ImageNet may not be necessary, or perhaps not even optimal, for model pretraining. We thus propose an unlabelled dataset PASS: Pictures without humAns for Self-Supervision. PASS only contains images with CC-BY license and complete attribution metadata, addressing the copyright issue. Most importantly, it contains no images of people at all, and also avoids other types of images that are problematic for data protection or ethics. We show that PASS can be used for pretraining with methods such as MoCo-v2, SwAV and DINO. In the transfer learning setting, it yields similar downstream performances to ImageNet pretraining even on tasks that involve humans, such as human pose estimation. PASS does not make existing datasets obsolete, as for instance it is insufficient for benchmarking. However, it shows that model pretraining is often possible while using safer data, and it also provides the basis for a more robust evaluation of pretraining methods.

==> 9_conclusion.tex <==
\section{Conclusion}

In the introduction, we have motivated our new dataset PASS from a scientific, ethical and legal perspective.
By using CC-BY images, we greatly reduce the risk of using images in a manner incompatible with copyright.
By avoiding the usage of search engines and labels to form a dataset, we avoid introducing corresponding biases.
By excluding all images that contain humans, as well as other identifiable information and NSFW images, we significantly reduce data protection and other ethics risks for the data subjects~\cite{prabhu20large}.
We have shown that, despite or because of these changes, we can effectively pre-train neural networks using this data.

However, several limitations remain.
First, while we put care in filtering the images, automatically and manually, some harmful content might have slipped through.

Second, sampled images randomly from an uncurated large collection removes specific biases such as search engine selection but not others.
Furthermore, we added one significant bias: there are no people in these pictures, despite the fact that the vast majority of images in existence contain people.
While this appears to be acceptable for model pretraining, \DSn cannot be used to learn models of people, such as for pose recognition.

Thirdly, pretraining on \DSn is equivalent to ImageNet or other such datasets only in the transfer learning setting.
Pretraining in a non-transfer learning setting is not very useful in applications, but is used for benchmarking.

Fourthly, since \DSn contains no labels, \DSn cannot be used alone for benchmarking.
For this, curated datasets remain necessary.
There is also the issue of reproducibility and model comparison: traditional benchmarks such as ImageNet are likely to remain essential to allow researchers to compare models.


Nonetheless, we believe that \DSn is an step towards curating and improving our dastasets to reduce scientific, ethical and legal risks for many tasks and applications.

==> tabs/splits_descriptions.tex <==
\begin{table}[t]
\caption{Pretraining data splits analyzed.}
  \centering
  \footnotesize   
    \setlength{\tabcolsep}{2pt}
  \begin{tabular}{l l}
    \toprule
    Dataset & Description \\
    \midrule
    \DSn             & Balanced user-contributions s.t. each user contributes  <80 images (avg. 14 per user).  \\
    \DSn\!-w/ humans & Same as above, but without filtering out humans. Shares 27\% of images with \DSn\!. \\
                     & Approx. 57\% of images contain humans.   \\
    \DSn\!-random    & A random split of 6M images.  \\
    \DSn\!-IN800     & Split generated to mimic IN-1k. An IN-1k pretrained classifier is run on our 6M images, and images    \\
                     & corresponding to the most frequent 800 classes are taken, s.t. each class has at most 2000 images. \\
    \DSn\!-6M        & All 6M images after cleaning that do not contain humans, as determined by pretrained models.  \\
  \bottomrule
  \end{tabular}
\end{table}

==> vedaldi.tex <==
\newif\ifdark
\IfFileExists{/Users/vedaldi/.bash_profile}{
\makeatletter
\immediate\write18{\unexpanded{%
if defaults read -g AppleInterfaceStyle 2>/dev/null;
then echo \\darktrue > /tmp/displaymode.tex;
else echo \\darkfalse > /tmp/displaymode.tex; fi}}
\makeatother 
\input{/tmp/displaymode.tex}
\ifdark
\definecolor{pcolor}{HTML}{1E1E1E}
\definecolor{tcolor}{HTML}{C5C5C5}
\else
\definecolor{pcolor}{HTML}{FDF6E3}
\definecolor{tcolor}{HTML}{333333}
\fi
\pagecolor{pcolor}
\color{tcolor}
% Suppress hbadness warnings.
\hbadness=\maxdimen
\vbadness=\maxdimen
\vfuzz=30pt
\hfuzz=30pt
}{} 

==> vedaldi_specific.tex <==
@STRING{accv    = {Proceedings of the {Asian Conference on Computer Vision}
                  ({ACCV})} }
@STRING{bmvc    = {Proceedings of the British Machine Vision Conference
                  ({BMVC})} }
@STRING{cvpr    = {Proceedings of the {IEEE} Conference on Computer Vision
                  and Pattern Recognition ({CVPR})} }
@STRING{cvprw   = {Proceedings of the {IEEE} Conference on Computer Vision
                  and Pattern Recognition Workshops ({CVPRW})} }
@STRING{eccv    = {Proceedings of the European Conference on Computer Vision
                  ({ECCV})} }
@STRING{icass   = {International Conference on Acoustics, Speech, and Signal
                  Processing (ICASS)} }
@STRING{iccv    = {Proceedings of the International Conference on Computer
                  Vision ({ICCV})} }
@STRING{iclr    = {Proceedings of the International Conference on Learning
                  Representations ({ICLR})} }
@STRING{icml    = {Proceedings of the International Conference on Machine
                  Learning ({ICML})} }
@STRING{ijcv    = {International Journal of Computer Vision ({IJCV})} }
@STRING{nips    = {Proceedings of Advances in Neural Information Processing
                  Systems (NeurIPS)} }
@STRING{pami    = {{IEEE} Transactions on Pattern Analysis and Machine
                  Intelligence} }

@InProceedings{ehrhardt20relate:,
  author     = {S{\'{e}}bastien Ehrhardt and Oliver Groth and Aron Monszpart
               and Martin Engelcke and Ingmar Posner and Niloy J. Mitra and
               Andrea Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {{RELATE:} Physically Plausible Multi-Object Scene Synthesis
               Using Structured Latent Spaces},
  year       = {2020}
}

@InProceedings{laina20quantifying,
  author     = {Iro Laina and Ruth C. Fong and Andrea Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {Quantifying Learnability and Describability of Visual
               Concepts Emerging in Representation Learning},
  year       = {2020}
}

@InProceedings{asano20labelling,
  author     = {Yuki M. Asano and Mandela Patrick and Christian Rupprecht and
               Andrea Vedaldi},
  booktitle  = nips,
  title      = {Labelling unlabelled videos from scratch with multi-modal
               self-supervision},
  year       = {2020}
}

@InProceedings{biggs203d-multi-bodies:,
  author     = {Benjamin Biggs and Andrea Vedaldi and David Novotn{\'{y}}},
  booktitle  = nips,
  title      = {{3D} Multi-bodies: Fitting Sets of Plausible {3D} Human
               Models to Ambiguous Image Data},
  year       = {2020}
}

@InProceedings{novotny20canonical,
  author     = {David Novotn{\'{y}} and Roman Shapovalov and Andrea Vedaldi},
  booktitle  = nips,
  title      = {Canonical {3D} Deformer Maps: Unifying parametric and
               non-parametric methods for dense weakly-supervised category
               reconstruction},
  year       = {2020}
}

@InProceedings{neverova20continuous,
  author     = {Natalia Neverova and David Novotn{\'{y}} and Andrea Vedaldi},
  booktitle  = nips,
  title      = {Continuous Surface Embeddings},
  year       = {2020}
}

@Article{ulyanov20deep,
  author     = {Dmitry Ulyanov and Andrea Vedaldi and Victor S. Lempitsky},
  journal    = ijcv,
  keywords   = {IDIU},
  number     = {7},
  pages      = {1867--1888},
  title      = {Deep Image Prior},
  volume     = {128},
  year       = {2020}
}

@InProceedings{chen20vggsound,
  author     = {Honglie Chen and Weidi Xie and Andrea Vedaldi and Andrew
               Zisserman},
  booktitle  = icass,
  title      = {{VGGSound}: A Large-scale Audio-Visual Dataset},
  year       = {2020}
}

@InProceedings{neumann19future,
  author     = {Luk{\'{a}}s Neumann and Andrew Zisserman and Andrea Vedaldi},
  booktitle  = cvprw,
  keywords   = {IDIU},
  title      = {Future Event Prediction: If and When},
  year       = {2019}
}

@InProceedings{sanakoyeu20transferring,
  author     = {Artsiom Sanakoyeu and Vasil Khalidov and Maureen S. McCarthy
               and Andrea Vedaldi and Natalia Neverova},
  booktitle  = cvpr,
  title      = {Transferring Dense Pose to Proximal Animal Classes},
  year       = {2020}
}

@InProceedings{jakab20self-supervised,
  author     = {Tomas Jakab and Ankush Gupta and Hakan Bilen and Andrea
               Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {Self-supervised Learning of Interpretable Keypoints from
               Unlabelled Videos},
  year       = {2020}
}

@InProceedings{wu20unsupervised,
  author     = {Shangzhe Wu and Christian Rupprecht and Andrea Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {Unsupervised Learning of Probably Symmetric Deformable {3D}
               Objects from Images in the Wild},
  url        = {https://elliottwu.com/projects/unsup3d/},
  year       = {2020}
}

@InProceedings{rebuffi20there,
  author     = {Sylvestre-Alvise Rebuffi and Ruth C. Fong and Xu Ji and
               Andrea Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {There and Back Again: Revisiting Backpropagation Saliency
               Methods},
  year       = {2020}
}

@InProceedings{han20automatically,
  author     = {Kai Han and Sylvestre-Alvise Rebuffi and Sebastien Ehrhardt
               and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = iclr,
  keywords   = {IDIU},
  title      = {Automatically Discovering and Learning New Visual Categories
               with Ranking Statistics},
  year       = {2020}
}

@InProceedings{asano20a-critical,
  author     = {Yuki M. Asano and Christian Rupprecht and Andrea Vedaldi},
  booktitle  = iclr,
  keywords   = {IDIU},
  title      = {A critical analysis of self-supervision, or what we can learn
               from a single image},
  year       = {2020}
}

@InProceedings{asano20self-labelling,
  author     = {Yuki M. Asano and Christian Rupprecht and Andrea Vedaldi},
  booktitle  = iclr,
  keywords   = {IDIU},
  title      = {Self-labelling via simultaneous clustering and representation
               learning},
  year       = {2020}
}

@Book{19explainable,
  editor     = {Wojciech Samek and Gr{\'{e}}goire Montavon and Andrea Vedaldi
               and Lars Kai Hansen and Klaus{-}Robert M{\"{u}}ller},
  keywords   = {IDIU},
  publisher  = {Springer},
  title      = {Explainable {AI:} Interpreting, Explaining and Visualizing
               Deep Learning},
  year       = {2019}
}

@InProceedings{touvron19fixing,
  author     = {Hugo Touvron and Andrea Vedaldi and Matthijs Douze and
               Herv{\'{e}} J{\'{e}}gou},
  booktitle  = nips,
  title      = {Fixing the train-test resolution discrepancy},
  year       = {2019}
}

@InProceedings{neverova19correlated,
  author     = {Natalia Neverova and David Novotn{\'{y}} and Andrea Vedaldi},
  booktitle  = nips,
  title      = {Correlated Uncertainty for Learning Dense Correspondences
               from Noisy Labels},
  year       = {2019}
}

@InProceedings{chen19autocorrect,
  author     = {Honglie Chen and Weidi Xie and Andrea Vedaldi and Andrew
               Zisserman},
  booktitle  = bmvc,
  title      = {{AutoCorrect}: Deep Inductive Alignment of Noisy Geometric
               Annotations},
  year       = {2019}
}

@InProceedings{neumann18relaxed,
  author     = {Luk{\'{a}}s Neumann and Andrew Zisserman and Andrea Vedaldi},
  booktitle  = {{NeurIPS} Workshop on Machine Learning for Intelligent
               Transportation Systems},
  title      = {Relaxed Softmax: Efficient Confidence Auto-Calibration for
               Safe Pedestrian Detection},
  year       = {2018}
}

@InProceedings{fuchs19scrutinizing,
  author     = {Fabian B. Fuchs and Oliver Groth and Adam R. Kosiorek and
               Alex Bewley and Markus Wulfmeier and Andrea Vedaldi and Ingmar
               Posner},
  booktitle  = bmvc,
  keywords   = {IDIU},
  title      = {Scrutinizing and De-Biasing Intuitive Physics with Neural
               Stethoscopes},
  year       = {2019}
}

@InProceedings{novotny19c3dpo,
  author     = {David Novotn{\'{y}} and Nikhila Ravi and Benjamin Graham and
               Natalia Neverova and Andrea Vedaldi},
  booktitle  = iccv,
  title      = {{C3DPO}: Canonical 3D Pose Networks for Non-Rigid Structure
               From Motion},
  year       = {2019}
}

@InProceedings{gupta18learning,
  author     = {Ankush Gupta and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = {Proceedings of the {Indian Conference on Computer Vision,
               Graphics and Image Processing}},
  title      = {Learning to read by spelling: Towards unsupervised text
               recognition},
  year       = {2018}
}

@InProceedings{henriques19small,
  author     = {Jo{\~{a}}o F. Henriques and S{\'{e}}bastien Ehrhardt and
               Samuel Albanie and Andrea Vedaldi},
  booktitle  = iccv,
  keywords   = {IDIU},
  title      = {Small step and giant leaps: Minimal {Netwon} solvers for Deep
               Learning},
  year       = {2019}
}

@InProceedings{thewlis19unsupervised,
  author     = {James Thewlis and Samuel Albanie and Hakan Bilen and Andrea
               Vedaldi},
  booktitle  = iccv,
  keywords   = {IDIU},
  title      = {Unsupervised learning of landmarks by descriptor vector
               exchange},
  year       = {2019}
}

@InProceedings{fong19understanding,
  author     = {Ruth Fong and Mandela Patrick and Andrea Vedaldi},
  booktitle  = iccv,
  title      = {Understanding Deep Networks via Extremal Perturbations and
               Smooth Masks},
  year       = {2019}
}

@InProceedings{ji19invariant,
  author     = {Xu Ji and Jo{\~{a}}o F. Henriques and Andrea Vedaldi},
  booktitle  = iccv,
  keywords   = {IDIU},
  title      = {Invariant Information Clustering for Unsupervised Image
               Classification and Segmentation},
  year       = {2019}
}

@InProceedings{han19learning,
  author     = {Kai Han and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = iccv,
  keywords   = {IDIU},
  title      = {Learning to Discover Novel Visual Categories via Deep
               Transfer Clustering},
  year       = {2019}
}

@Article{balntas19hpatches,
  author     = {Vassileios Balntas and Karel Lenc and Andrea Vedaldi and
               Tinne Tuytelaars and Jiri Matas and Krystian Mikolajczyk},
  journal    = pami,
  keywords   = {IDIU},
  title      = {{HPatches}: A benchmark and evaluation of handcrafted and
               learned local descriptors},
  year       = {2019}
}

@Article{ehrhardt19taking,
  author     = {S{\'{e}}bastien Ehrhardt and Aron Monszpart and Niloy J.
               Mitra and Andrea Vedaldi},
  journal    = {Computer Vision and Image Understanding},
  keywords   = {IDIU},
  title      = {Taking visual motion prediction to new heightfields},
  year       = {2019}
}

@Article{novotny18capturing,
  author     = {David Novotn{\'{y}} and Diane Larlus and Andrea Vedaldi},
  journal    = pami,
  keywords   = {IDIU},
  title      = {Capturing the Geometry of Object Categories from Video
               Supervision},
  year       = {2018}
}

@InProceedings{bertinetto19meta-learning,
  author     = {Luca Bertinetto and Jo{\~{a}}o F. Henriques and Philip H. S.
               Torr and Andrea Vedaldi},
  booktitle  = iclr,
  keywords   = {IDIU},
  title      = {Meta-learning with differentiable closed-form solvers},
  url        = {https://www.robots.ox.ac.uk/~luca/r2d2.html},
  year       = {2019}
}

@InProceedings{neverova19slim,
  author     = {Natalia Neverova and James Thewlis and Riza Alp G{\"{u}}ler
               and Iasonas Kokkinos and Andrea Vedaldi},
  booktitle  = cvpr,
  title      = {Slim {DensePose}: Thrifty Learning From Sparse Annotations
               and Motion Cues},
  year       = {2019}
}

@InProceedings{ehrhardt18unsupervised,
  author     = {S{\'{e}}bastien Ehrhardt and Aron Monszpart and Niloy J.
               Mitra and Andrea Vedaldi},
  booktitle  = accv,
  keywords   = {IDIU},
  title      = {Unsupervised Intuitive Physics from Visual Observations},
  year       = {2018}
}

@InProceedings{neumann18nightowls,
  author     = {Luk{\'{a}}s Neumann and Michelle Karg and Shanshan Zhang and
               Christian Scharfenberger and Eric Piegert and Sarah Mistr and
               Olga Prokofyeva and Robert Thiel and Andrea Vedaldi and Andrew
               Zisserman and Bernt Schiele},
  booktitle  = accv,
  title      = {{NightOwls}: {A} Pedestrians at Night Dataset},
  year       = {2018}
}

@InProceedings{neumann18tiny,
  author     = {Luk{\'{a}}s Neumann and Andrea Vedaldi},
  booktitle  = accv,
  title      = {Tiny People Pose},
  year       = {2018}
}

@InProceedings{mahendran18cross,
  author     = {Aravindh Mahendran and James Thewlis and Andrea Vedaldi},
  booktitle  = accv,
  keywords   = {IDIU},
  title      = {Cross Pixel Optical-Flow Similarity for Self-supervised
               Learning},
  year       = {2018}
}

@InProceedings{albanie18emotion,
  author     = {Samuel Albanie and Arsha Nagrani and Andrea Vedaldi and
               Andrew Zisserman},
  booktitle  = {Proceedings of the 26th annual {ACM} international conference
               on Multimedia},
  title      = {Emotion Recognition in Speech using Cross-Modal Transfer in
               the Wild},
  year       = {2018}
}

@InProceedings{jakab18unsupervised,
  author     = {Tomas Jakab and Ankush Gupta and Hakan Bilen and Andrea
               Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {Unsupervised Learning of Object Landmarks through Conditional
               Image Generation},
  year       = {2018}
}

@InProceedings{thewlis18modelling,
  author     = {James Thewlis and Hakan Bilen and Andrea Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {Modelling and unsupervised learning of symmetric deformable
               object categories},
  year       = {2018}
}

@InProceedings{hu18gather,
  author     = {Jie Hu and Li Shen and Samuel Albanie and Gang Sun and Andrea
               Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {Gather-Excite: Exploiting Feature Context in Convolutional
               Neural Networks},
  year       = {2018}
}

@InProceedings{gupta18inductive,
  author     = {Ankush Gupta and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = bmvc,
  title      = {Inductive Visual Localisation: Factorised Training for
               Superior Generalisation},
  year       = {2018}
}

@InProceedings{valmadre18long-term,
  author     = {Jack Valmadre and Luca Bertinetto and Jo{\~{a}}o F. Henriques
               and Ran Tao and Andrea Vedaldi and Arnold W. M. Smeulders and
               Philip H. S. Torr and Efstratios Gavves},
  booktitle  = eccv,
  title      = {Long-Term Tracking in the Wild: {A} Benchmark},
  year       = {2018}
}

@InProceedings{klodt18supervising,
  author     = {Maria Klodt and Andrea Vedaldi},
  booktitle  = eccv,
  title      = {Supervising the New with the Old: Learning {SFM} from {SFM}},
  year       = {2018}
}

@InProceedings{lenc18large,
  author     = {Karel Lenc and Andrea Vedaldi},
  booktitle  = bmvc,
  keywords   = {IDIU},
  title      = {Large scale evaluation of local image feature detectors on
               homography datasets},
  year       = {2018}
}

@InProceedings{groth18shapestacks,
  author     = {Oliver Groth and Fabian B. Fuchs and Ingmar Posner and Andrea
               Vedaldi},
  booktitle  = eccv,
  keywords   = {IDIU},
  title      = {{ShapeStacks}: Learning Vision-Based Physical Intuition for
               Generalised Object Stacking},
  url        = {https://shapestacks.robots.ox.ac.uk},
  year       = {2018}
}

@InProceedings{novotny18semi-convolutional,
  author     = {David Novotn{\'{y}} and Samuel Albanie and Diane Larlus and
               Andrea Vedaldi},
  booktitle  = eccv,
  keywords   = {IDIU},
  title      = {Semi-convolutional Operators for Instance Segmentation},
  year       = {2018}
}

@Article{lenc18understanding,
  author     = {Karel Lenc and Andrea Vedaldi},
  journal    = ijcv,
  keywords   = {IDIU},
  number     = {5},
  title      = {Understanding Image Representations by Measuring Their
               Equivariance and Equivalence},
  volume     = {127},
  year       = {2019}
}

@InProceedings{fong18net2vec,
  author     = {Ruth Fong and Andrea Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {{Net2Vec}: Quantifying and Explaining How Concepts Are
               Encoded by Filters in Deep Neural Networks},
  year       = {2018}
}

@InProceedings{henriques18mapnet,
  author     = {Jo{\~{a}}o F. Henriques and Andrea Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {{MapNet}: An Allocentric Spatial Memory for Mapping
               Environments},
  year       = {2018}
}

@InProceedings{rebuffi18efficient,
  author     = {Sylvestre{-}Alvise Rebuffi and Hakan Bilen and Andrea
               Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {Efficient Parametrization of Multi-Domain Deep Neural
               Networks},
  url        = {https://github.com/srebuffi/residual_adapters},
  year       = {2018}
}

@InProceedings{novotny18self-supervised,
  author     = {David Novotn{\'{y}} and Samuel Albanie and Diane Larlus and
               Andrea Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {Self-Supervised Learning of Geometrically Stable Features
               Through Probabilistic Introspection},
  year       = {2018}
}

@InProceedings{ulyanov18deep,
  author     = {Dmitry Ulyanov and Andrea Vedaldi and Victor S. Lempitsky},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {Deep Image Prior},
  url        = {https://dmitryulyanov.github.io/deep_image_prior},
  year       = {2018}
}

@InCollection{novotny17generalizing,
  author     = {David Novotn{\'{y}} and Diane Larlus and Andrea Vedaldi},
  booktitle  = {Domain Adaptation in Computer Vision Applications},
  pages      = {259--273},
  publisher  = {Springer, Cham},
  title      = {Generalizing Semantic Part Detectors Across Domains},
  year       = {2017}
}

@InProceedings{ulyanov18takes,
  author     = {Dmitry Ulyanov and Andrea Vedaldi and Victor S. Lempitsky},
  booktitle  = {Proceedings of the Association for the Advancement of
               Artificial Intelligence ({AAAI})},
  keywords   = {IDIU},
  title      = {It Takes {(Only)} Two: Adversarial Generator-Encoder
               Networks},
  year       = {2018}
}

@Article{bilen18action,
  author     = {Hakan Bilen and Basura Fernando and Efstratios Gavves and
               Andrea Vedaldi},
  journal    = pami,
  keywords   = {IDIU},
  number     = {12},
  title      = {Action Recognition with Dynamic Image Networks},
  volume     = {40},
  year       = {2018}
}

@InProceedings{thewlis17dense,
  author     = {James Thewlis and Hakan Bilen and Andrea Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {Unsupervised learning of object frames by dense equivariant
               image labelling},
  year       = {2017}
}

@InProceedings{rebuffi17learning,
  author     = {Sylvestre{-}Alvise Rebuffi and Hakan Bilen and Andrea
               Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {Learning multiple visual domains with residual adapters},
  url        = {https://github.com/srebuffi/residual_adapters},
  year       = {2017}
}

@InProceedings{novotny17learning,
  author     = {David Novotn{\'{y}} and Diane Larlus and Andrea Vedaldi},
  booktitle  = iccv,
  keywords   = {IDIU},
  title      = {Learning {3D} Object Categories by Looking Around Them},
  year       = {2017}
}

@InProceedings{fong17interpretable,
  author     = {Ruth C. Fong and Andrea Vedaldi},
  booktitle  = iccv,
  keywords   = {IDIU},
  title      = {Interpretable Explanations of Black Boxes by Meaningful
               Perturbation},
  year       = {2017}
}

@InProceedings{thewlis17unsupervised,
  author     = {James Thewlis and Hakan Bilen and Andrea Vedaldi},
  booktitle  = iccv,
  keywords   = {IDIU},
  title      = {Unsupervised Learning of Object Landmarks by Factorized
               Spatial Embeddings},
  year       = {2017}
}

@InProceedings{henriques17warped,
  author     = {Jo{\~{a}}o F. Henriques and Andrea Vedaldi},
  booktitle  = icml,
  keywords   = {IDIU},
  title      = {Warped Convolutions: Efficient Invariance to Spatial
               Transformations},
  year       = {2017}
}

@InProceedings{bertinetto17end-to-end,
  author     = {Jack Valmadre and Luca Bertinetto and Jo{\~{a}}o F. Henriques
               and Andrea Vedaldi and Philip H. S. Torr},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {End-to-End Representation Learning for Correlation Filter
               Based Tracking},
  year       = {2017}
}

@InProceedings{bertinetto16fully,
  author     = {Luca Bertinetto and Jack Valmadre and Jo{\~{a}}o F. Henriques
               and Andrea Vedaldi and Philip H. S. Torr},
  booktitle  = {{ECCV} Workshop on Computer Vision on Visual Object
               Tracking},
  keywords   = {IDIU},
  title      = {Fully-Convolutional Siamese Networks for Object Tracking},
  year       = {2016}
}

@InProceedings{ulyanov17improved,
  author     = {Dmitry Ulyanov and Andrea Vedaldi and Victor S. Lempitsky},
  booktitle  = cvpr,
  title      = {Improved Texture Networks: Maximizing Quality and Diversity
               in Feed-Forward Stylization and Texture Synthesis},
  year       = {2017}
}

@InProceedings{novotny17anchornet,
  author     = {David Novotn{\'{y}} and Diane Larlus and Andrea Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {{AnchorNet}: {A} Weakly Supervised Network to Learn
               Geometry-Sensitive Features for Semantic Matching},
  year       = {2017}
}

@InProceedings{balntas17hpatch,
  author     = {Vassileios Balntas and Karel Lenc and Andrea Vedaldi and
               Krystian Mikolajczyk},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {{HPatches}: {A} Benchmark and Evaluation of Handcrafted and
               Learned Local Descriptors},
  year       = {2017}
}

@InProceedings{lenc16learning,
  author     = {Karel Lenc and Andrea Vedaldi},
  booktitle  = {Proceedings of the {ECCV} workshop on {Geometry Meets Deep
               Learning}},
  keywords   = {IDIU},
  title      = {Learning Covariant Feature Detectors},
  url        = {https://github.com/lenck/ddet},
  year       = {2016}
}

@InProceedings{novotny16learning,
  author     = {David Novotn{\'{y}} and Diane Larlus and Andrea Vedaldi},
  booktitle  = {Proceedings of the {ECCV} workshop on {Geometry Meets Deep
               Learning}},
  keywords   = {IDIU},
  title      = {Learning the semantic structure of objects from Web
               supervision},
  year       = {2016}
}

@InProceedings{bertinetto16learning,
  author     = {Luca Bertinetto and Jo{\~{a}}o F. Henriques and Jack Valmadre
               and Philip H. S. Torr and Andrea Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {Learning feed-forward one-shot learners},
  year       = {2016}
}

@InProceedings{bilen16integrated,
  author     = {Hakan Bilen and Andrea Vedaldi},
  booktitle  = nips,
  keywords   = {IDIU},
  title      = {Integrated perception with recurrent multi-task neural
               networks},
  year       = {2016}
}

@InProceedings{mahendran16salient,
  author     = {Aravindh Mahendran and Andrea Vedaldi},
  booktitle  = eccv,
  keywords   = {IDIU},
  title      = {Salient Deconvolutional Networks},
  year       = {2016}
}

@InProceedings{novotny16i-have,
  author     = {David Novotn{\'{y}} and Diane Larlus and Andrea Vedaldi},
  booktitle  = bmvc,
  keywords   = {IDIU},
  title      = {I Have Seen Enough: Transferring Parts Across Categories},
  year       = {2016}
}

@InProceedings{thewlis16fully-trainable,
  author     = {James Thewlis and Shuai Zheng and Philip H. S. Torr and
               Andrea Vedaldi},
  booktitle  = bmvc,
  keywords   = {IDIU},
  title      = {Fully-trainable deep matching},
  year       = {2016}
}

@InProceedings{albanie16learning,
  author     = {Samuel Albanie and Andrea Vedaldi},
  booktitle  = bmvc,
  keywords   = {IDIU},
  title      = {Learning Grimaces by Watching {TV}},
  url        = {http://www.robots.ox.ac.uk/~vgg/data/facevalue},
  year       = {2016}
}

@Article{gonfaus15factorized,
  author     = {Josep M. Gonfaus and Marco Pedersoli and Jordi Gonz{\`{a}}lez
               and Andrea Vedaldi and F. Xavier Roca},
  journal    = {Computer Vision and Image Understanding},
  pages      = {92--101},
  title      = {Factorized appearances for object detection},
  volume     = {138},
  year       = {2015}
}

@Article{mahendran16visualizing,
  author     = {Aravindh Mahendran and Andrea Vedaldi},
  journal    = ijcv,
  keywords   = {IDIU},
  number     = {3},
  title      = {Visualizing Deep Convolutional Neural Networks Using Natural
               Pre-images},
  volume     = {120},
  year       = {2016}
}

@InProceedings{ulyanov16texture,
  author     = {Dmitry Ulyanov and Vadim Lebedev and Andrea Vedaldi and
               Victor S. Lempitsky},
  booktitle  = icml,
  title      = {Texture Networks: Feed-forward Synthesis of Textures and
               Stylized Images},
  url        = {http://likemo.net/},
  year       = {2016}
}

@InProceedings{gupta16synthetic,
  author     = {Ankush Gupta and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = cvpr,
  title      = {Synthetic Data for Text Localisation in Natural Images},
  year       = {2016}
}

@InProceedings{bilen16dynamic,
  author     = {Hakan Bilen and Basura Fernando and Efstratios Gavves and
               Andrea Vedaldi and Stephen Gould},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {Dynamic Image Networks for Action Recognition},
  year       = {2016}
}

@InProceedings{bilen16weakly,
  author     = {Hakan Bilen and Andrea Vedaldi},
  booktitle  = cvpr,
  keywords   = {IDIU},
  title      = {Weakly Supervised Deep Detection Networks},
  year       = {2016}
}

@Article{cimpoi16deep,
  author     = {Mircea Cimpoi and Subhransu Maji and Iasonas Kokkinos and
               Andrea Vedaldi},
  journal    = ijcv,
  keywords   = {IDIU},
  number     = {1},
  title      = {Deep Filter Banks for Texture Recognition, Description, and
               Segmentation},
  volume     = {118},
  year       = {2016}
}

@InProceedings{parkhi15deep,
  author     = {Omkar M. Parkhi and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = bmvc,
  title      = {Deep Face Recognition},
  year       = {2015}
}

@InProceedings{vedaldi15matconvnet,
  author     = {Andrea Vedaldi and Karel Lenc},
  booktitle  = {Proceedings of the 25th annual {ACM} international conference
               on Multimedia},
  title      = {{MatConvNet}: Convolutional Neural Networks for {MATLAB}},
  year       = {2015}
}

@Article{jaderberg15reading,
  author     = {Max Jaderberg and Karen Simonyan and Andrea Vedaldi and
               Andrew Zisserman},
  journal    = ijcv,
  number     = {1},
  title      = {Reading Text in the Wild with Convolutional Neural Networks},
  volume     = {116},
  year       = {2016}
}

@InProceedings{lenc15rcnn,
  author     = {Karel Lenc and Andrea Vedaldi},
  booktitle  = bmvc,
  title      = {{R-CNN} minus {R}},
  year       = {2015}
}

@InProceedings{parizi15automatic,
  author     = {Sobhan Naderi Parizi and Andrea Vedaldi and Andrew Zisserman
               and Pedro F. Felzenszwalb},
  booktitle  = iclr,
  title      = {Automatic Discovery and Optimization of Parts for Image
               Classification},
  year       = {2015}
}

@InProceedings{cimpoi15deep,
  author     = {Mircea Cimpoi and Subhransu Maji and Andrea Vedaldi},
  booktitle  = cvpr,
  title      = {Deep filter banks for texture recognition and segmentation},
  url        = {http://www.robots.ox.ac.uk/~vgg/data/dtd/},
  year       = {2015}
}

@InProceedings{lenc15understanding,
  author     = {Karel Lenc and Andrea Vedaldi},
  booktitle  = cvpr,
  title      = {Understanding image representations by measuring their
               equivariance and equivalence},
  year       = {2015}
}

@InProceedings{mahendran15understanding,
  author     = {Aravindh Mahendran and Andrea Vedaldi},
  booktitle  = cvpr,
  title      = {Understanding deep image representations by inverting them},
  year       = {2015}
}

@InCollection{vedaldi10knowing,
  author     = {Andrea Vedaldi and Haibin Ling and Stefano Soatto},
  booktitle  = {Computer Vision: Detection, Recognition and Reconstruction},
  pages      = {27-49},
  publisher  = {Springer},
  title      = {Knowing a Good Feature When You See It: Ground Truth and
               Methodology to Evaluate Local Features for Recognition},
  volume     = {285},
  year       = {2010}
}

@Article{pedersoli14coarse,
  author     = {Marco Pedersoli and Andrea Vedaldi and Jordi Gonz{\`{a}}lez
               and F. Xavier Roca},
  journal    = {Pattern Recognition},
  title      = {A coarse-to-fine approach for fast deformable object
               detection},
  year       = {2014}
}

@InProceedings{jaderberg14synthetic,
  author     = {M. Jaderberg and K. Simonyan and Andrea Vedaldi and A.
               Zisserman},
  booktitle  = {{NeurIPS} Deep Learning Workshop},
  title      = {Synthetic Data and Artificial Neural Networks for Natural
               Scene Text Recognition},
  year       = {2014}
}

@InProceedings{jaderberg14deep,
  author     = {Max Jaderberg and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = eccv,
  title      = {Deep Features for Text Spotting},
  year       = {2014}
}

@InProceedings{chatfield14return,
  author     = {Ken Chatfield and Karen Simonyan and Andrea Vedaldi and
               Andrew Zisserman},
  booktitle  = bmvc,
  title      = {Return of the Devil in the Details: Delving Deep into
               Convolutional Nets},
  url        = {http://www.robots.ox.ac.uk/~vgg/research/deep_eval/},
  year       = {2014}
}

@InProceedings{jaderberg14speeding,
  author     = {Max Jaderberg and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = bmvc,
  title      = {Speeding up Convolutional Neural Networks with Low Rank
               Expansions},
  year       = {2014}
}

@InProceedings{vedaldi14understanding,
  author     = {Andrea Vedaldi and Siddharth Mahendran and Stavros Tsogkas
               and Subhransu Maji and Ross B. Girshick and Juho Kannala and
               Esa Rahtu and Iasonas Kokkinos and Matthew B. Blaschko and
               David J. Weiss and Ben Taskar and Karen Simonyan and Naomi
               Saphra and Sammy Mohamed},
  booktitle  = cvpr,
  title      = {Understanding Objects in Detail with Fine-Grained
               Attributes},
  url        = {http://www.robots.ox.ac.uk/~vgg/data/oid/},
  year       = {2014}
}

@InProceedings{cimpoi14describing,
  author     = {Mircea Cimpoi and Subhransu Maji and Iasonas Kokkinos and
               Sammy Mohamed and Andrea Vedaldi},
  booktitle  = cvpr,
  title      = {Describing Textures in the Wild},
  url        = {http://www.robots.ox.ac.uk/~vgg/data/dtd/},
  year       = {2014}
}

@InProceedings{parkhi14compact,
  author     = {Omkar M. Parkhi and Karen Simonyan and Andrea Vedaldi and
               Andrew Zisserman},
  booktitle  = cvpr,
  title      = {A Compact and Discriminative Face Track Descriptor},
  year       = {2014}
}

@InProceedings{simonyan14deep,
  author     = {Karen Simonyan and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = {Proceedings of the International Conference on Learning
               Representations ({ICLR})},
  title      = {Deep Inside Convolutional Networks: Visualising Image
               Classification Models and Saliency Maps},
  year       = {2014}
}

@Article{simonyan14learning,
  author     = {Karen Simonyan and Andrea Vedaldi and Andrew Zisserman},
  journal    = pami,
  number     = {8},
  title      = {Learning Local Feature Descriptors Using Convex
               Optimisation},
  volume     = {36},
  year       = {2014}
}

@InProceedings{simonyan13deep,
  author     = {Karen Simonyan and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = nips,
  title      = {Deep Fisher Networks for Large-Scale Image Classification},
  url        = {http://www.robots.ox.ac.uk/~vgg/software/face_desc/},
  year       = {2013}
}

@InProceedings{simonyan13fisher,
  author     = {Karen Simonyan and Omkar M. Parkhi and Andrea Vedaldi and
               Andrew Zisserman},
  booktitle  = bmvc,
  title      = {Fisher Vector Faces in the Wild},
  year       = {2013}
}

@InProceedings{juneja13blocks,
  author     = {Mayank Juneja and Andrea Vedaldi and C. V. Jawahar and Andrew
               Zisserman},
  booktitle  = cvpr,
  title      = {Blocks That Shout: Distinctive Parts for Scene
               Classification},
  year       = {2013}
}

@InProceedings{vedaldi12self,
  author     = {Andrea Vedaldi and Andrew Zisserman},
  booktitle  = eccv,
  title      = {Self-similar Sketch},
  year       = {2012}
}

@InProceedings{simonyan12descriptor,
  author     = {Karen Simonyan and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = eccv,
  title      = {Descriptor Learning Using Convex Optimisation},
  year       = {2012}
}

@InProceedings{parkhi12spotting,
  author     = {Omkar M. Parkhi and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = {Proceedings of the Int. Workshop on Image Analysis for
               Multimedia Interactive Services},
  title      = {On-the-fly specific person retrieval},
  year       = {2012}
}

@InProceedings{vedaldi12sparse,
  author     = {Andrea Vedaldi and Andrew Zisserman},
  booktitle  = cvpr,
  title      = {Sparse kernel approximations for efficient classification and
               detection},
  year       = {2012}
}

@InProceedings{parkhi12cat,
  author     = {Omkar M. Parkhi and Andrea Vedaldi and Andrew Zisserman and
               C. V. Jawahar},
  booktitle  = cvpr,
  title      = {Cats and dogs},
  year       = {2012}
}

@InProceedings{lempitsky11pylon,
  author     = {Victor S. Lempitsky and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = nips,
  title      = {Pylon Model for Semantic Segmentation},
  year       = {2011}
}

@InProceedings{chatfield11devil,
  author     = {Ken Chatfield and Victor S. Lempitsky and Andrea Vedaldi and
               Andrew Zisserman},
  booktitle  = bmvc,
  title      = {The devil is in the details: an evaluation of recent feature
               encoding methods},
  url        = {http://www.robots.ox.ac.uk/~vgg/research/encoding_eval/},
  year       = {2011}
}

@InProceedings{parkhi11truth,
  author     = {Omkar M. Parkhi and Andrea Vedaldi and C. V. Jawahar and
               Andrew Zisserman},
  booktitle  = iccv,
  title      = {The truth about cats and dogs},
  year       = {2011}
}

@InProceedings{vedaldi11learning,
  author     = {Andrea Vedaldi and Matthew B. Blaschko and Andrew Zisserman},
  booktitle  = iccv,
  title      = {Learning equivariant structured output {SVM} regressors},
  year       = {2011}
}

@Article{vedaldi11efficient,
  author     = {Andrea Vedaldi and Andrew Zisserman},
  journal    = pami,
  number     = {3},
  title      = {Efficient Additive Kernels via Explicit Feature Maps},
  volume     = {34},
  year       = {2012}
}

@InProceedings{pedersoli11coarse,
  author     = {Marco Pedersoli and Andrea Vedaldi and Jordi Gonz{\`{a}}lez},
  booktitle  = cvpr,
  title      = {A coarse-to-fine approach for fast deformable object
               detection},
  year       = {2011}
}

@InProceedings{vedaldi10vlfeat,
  author     = {Andrea Vedaldi and Brian Fulkerson},
  booktitle  = {Proceedings of the 18th annual {ACM} international conference
               on Multimedia},
  title      = {{VLFeat}: an open and portable library of computer vision
               algorithms},
  year       = {2010}
}

@InProceedings{blaschko10simultaneous,
  author     = {Matthew B. Blaschko and Andrea Vedaldi and Andrew Zisserman},
  booktitle  = nips,
  title      = {Simultaneous Object Detection and Ranking with Weak
               Supervision},
  year       = {2010}
}

@InProceedings{vempati10generalized,
  author     = {Sreekanth Vempati and Andrea Vedaldi and Andrew Zisserman and
               C. V. Jawahar},
  booktitle  = bmvc,
  title      = {Generalized {RBF} feature maps for Efficient Detection},
  year       = {2010}
}

@InProceedings{vedaldi10efficient,
  author     = {Andrea Vedaldi and Andrew Zisserman},
  booktitle  = cvpr,
  title      = {Efficient additive kernels via explicit feature maps},
  year       = {2010}
}

@InProceedings{vedaldi09structured,
  author     = {Andrea Vedaldi and A. Zisserman},
  booktitle  = nips,
  title      = {Structured output regression for detection with partial
               occulsion},
  year       = {2009}
}

@InProceedings{vedaldi09multiple,
  author     = {Andrea Vedaldi and Varun Gulshan and Manik Varma and Andrew
               Zisserman},
  booktitle  = iccv,
  title      = {Multiple kernels for object detection},
  year       = {2009}
}

@InProceedings{fulkerson09class,
  author     = {Brian Fulkerson and Andrea Vedaldi and Stefano Soatto},
  booktitle  = iccv,
  title      = {Class segmentation and object localization with superpixel
               neighborhoods},
  year       = {2009}
}

@InProceedings{fulkerson08localizing,
  author     = {Brian Fulkerson and Andrea Vedaldi and Stefano Soatto},
  booktitle  = eccv,
  title      = {Localizing Objects with Smart Dictionaries},
  year       = {2008}
}

@InProceedings{vedaldi08quick,
  author     = {Andrea Vedaldi and Stefano Soatto},
  booktitle  = eccv,
  title      = {Quick Shift and Kernel Methods for Mode Seeking},
  year       = {2008}
}

@InProceedings{vedaldi08relaxed,
  author     = {Andrea Vedaldi and Stefano Soatto},
  booktitle  = cvpr,
  title      = {Relaxed Matching Kernels for Object Recognition},
  year       = {2008}
}

@InProceedings{vedaldi08joint,
  author     = {Andrea Vedaldi and Gregorio Guidi and Stefano Soatto},
  booktitle  = cvpr,
  title      = {Joint data alignment up to (lossy) transformations},
  year       = {2008}
}

@InProceedings{rabinovich07objects,
  author     = {Andrew Rabinovich and Andrea Vedaldi and Carolina
               Galleguillos and Eric Wiewiora and Serge J. Belongie},
  booktitle  = iccv,
  title      = {Objects in Context},
  year       = {2007}
}

@InProceedings{vedaldi07boosting,
  author     = {Andrea Vedaldi and Paolo Favaro and Enrico Grisan},
  booktitle  = iccv,
  title      = {Boosting Invariance and Efficiency in Supervised Learning},
  year       = {2007}
}

@InProceedings{vedaldi07moving,
  author     = {Andrea Vedaldi and Gregorio Guidi and Stefano Soatto},
  booktitle  = cvpr,
  title      = {Moving Forward in Structure From Motion},
  year       = {2007}
}

@InProceedings{jones07inertial,
  author     = {Eagle Jones and Andrea Vedaldi and Stefano Soatto},
  booktitle  = {Proceedings of {ICCV} Workshop on Dynamical Vision},
  title      = {Inertial structure from motion with autocalibration},
  year       = {2007}
}

@InProceedings{vedaldi07complexity,
  author     = {Andrea Vedaldi and Stefano Soatto},
  booktitle  = {Proceedings of Advances in Neural Information Processing
               Systems ({NeurIPS})},
  title      = {A Complexity-Distrotion Approach to Joint Pattern Alignment},
  year       = {2007}
}

@InProceedings{vedaldi06local,
  author     = {Andrea Vedaldi and Stefano Soatto},
  booktitle  = cvpr,
  title      = {Local Features, All Grown Up},
  year       = {2006}
}

@InProceedings{vedaldi06viewpoint,
  author     = {Andrea Vedaldi and Stefano Soatto},
  booktitle  = eccv,
  pages      = {374},
  title      = {Viewpoint Induced Deformation Statistics and the Design of
               Viewpoint Invariant Features: Singularities and Occlusions},
  year       = {2006}
}

@InProceedings{vedaldi05features,
  author     = {Andrea Vedaldi and Stefano Soatto},
  booktitle  = iccv,
  title      = {Features for Recognition: Viewpoint Invariance for Non-Planar
               Scenes},
  year       = {2005}
}

@InProceedings{vedaldi05kalmansac,
  author     = {Andrea Vedaldi and Hailin Jin and Paolo Favaro and Stefano
               Soatto},
  booktitle  = iccv,
  title      = {{KALMANSAC:} Robust Filtering by Consensus},
  year       = {2005}
}

@PhDThesis{vedaldi08invariant,
  author     = {Andrea Vedaldi},
  school     = {University of California at Los Angeles},
  title      = {Invariant Representations and Learning for Computer Vision},
  year       = {2008}
}

@TechReport{vedaldi07open,
  author     = {Andrea Vedaldi},
  institution= {{UCLA CSD}},
  number     = {070012},
  title      = {An open implementation of the {SIFT} detector and
               descriptor},
  year       = {2007}
}

@TechReport{vedaldiTR05viewpoint,
  author     = {Andrea Vedaldi and Stefano Soatto},
  institution= {{UCLA} {CSD}},
  number     = {050012},
  title      = {On Viewpoint Invariance for Non-Planar Scenes},
  year       = {2005}
}

